XP-MARL: Auxiliary Prioritization in Multi-Agent Reinforcement Learning to Address Non-Stationarity

Non-stationarity poses a fundamental challenge in Multi-Agent Reinforcement Learning (MARL), arising from agents simultaneously learning and altering their policies. This creates a non-stationary environment from the perspective of each individual agent, often leading to suboptimal or even unconverged learning outcomes. We propose an open-source framework named XP-MARL, which augments MARL with auxiliary prioritization to address this challenge in cooperative settings. XP-MARL is 1) founded upon our hypothesis that prioritizing agents and letting higher-priority agents establish their actions first would stabilize the learning process and thus mitigate non-stationarity and 2) enabled by our proposed mechanism called action propagation, where higher-priority agents act first and communicate their actions, providing a more stationary environment for others. Moreover, instead of using a predefined or heuristic priority assignment, XP-MARL learns priority-assignment policies with an auxiliary MARL problem, leading to a joint learning scheme. Experiments in a motion-planning scenario involving Connected and Automated Vehicles (CAVs) demonstrate that XP-MARL improves the safety of a baseline model by 84.4% and outperforms a state-of-the-art approach, which improves the baseline by only 12.8%. Code: github.com/cas-lab-munich/sigmarl

==> copyright.tex <==
\def\doi{10.23919/ECC54610.2021.9654986}% <--- Change here

\ifpreprint
    \makeatletter
    \def\ps@IEEEtitlepagestyle{%
        \def\@oddfoot{\mycopyrightnotice}%
        \def\@evenfoot{}%
    }
    \ifpublished
        \def\mycopyrightnotice{%
            \begin{minipage}{\textwidth}
                \centering \scriptsize
                \href{https://doi.org/\doi}{DOI: \doi} \copyright \the\year{} IEEE. Personal use of this material is permitted. Permission from IEEE must be obtained for all other uses, in any current or future media, including reprinting/republishing this material for advertising or promotional purposes, creating new collective works, for resale or redistribution to servers or lists, or reuse of any copyrighted component of this work in other works.\hfill% <--- Change here
            \end{minipage}
            \gdef\mycopyrightnotice{}% just in case
        }
    \else% preprint, submitted
        \def\mycopyrightnotice{%
            \begin{minipage}{\textwidth}
                \centering \scriptsize
                This work has been submitted to the IEEE for possible publication. Copyright may be transferred without notice, after which this version may no longer be accessible.
            \end{minipage}
            \gdef\mycopyrightnotice{}% just in case
        }
    \fi
    \makeatother
\fi
